AI Alignment From Social Choice Perspectives

Alignment from human feedback uses human judgments about model outputs to steer the behavior of language models after pretraining. When those judgments reflect conflicting views of desirable behavior, the learned objective becomes an aggregate determination of what the model should prefer. We survey recent work that has studied this aggregation problem through the lens of social choice theory. We illustrate how the social choice perspective helps identify failure modes in the feedback aggregation layer and reveals a broader design space for handling disagreement in explicit and principled ways.

==> style/macros.tex <==

\definecolor{highlightcolor}{HTML}{e9f1ff}
\definecolor{custombar}{HTML}{aadbc9}
\definecolor{newtext}{rgb}{0.1,0.3,0.4}

\makeatletter
\@ifundefined{newdef}{\let\newdef\newtheorem}{}
\makeatother

\newtheorem{theorem}{Theorem}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{assumption}[theorem]{Assumption}
\newdef{definition}[theorem]{Definition}
\newdef{remark}[theorem]{Remark}

\makeatletter
\providecommand*{\theHtheorem}{\arabic{theorem}}

\newcommand{\scai@begintheorem}[2]{\refstepcounter{theorem}\begingroup
    \edef\x{\endgroup
      \noexpand\gdef\noexpand\scai@theoremhref{\@currentHref}}\x
  \trivlist
  \item[\hskip 10pt\hskip\labelsep{{\normalfont\scshape Theorem}\hskip 5pt\relax \thetheorem\if\relax\detokenize{#1}\relax
      .\else
      \hskip 5pt\relax #1.\fi
  }]\itshape
  \let\@currentHref\scai@theoremhref
  \ignorespaces
}
\renewenvironment{theorem}[1][]{\scai@begintheorem{#1}{}}{\endtrivlist}

\def\@begintheorem#1#2{\trivlist \item[\hskip 10pt\hskip
\labelsep{{\normalfont\scshape #1}\hskip 5pt\relax #2.}] \itshape}
\def\@opargbegintheorem#1#2#3{\trivlist
\item[\hskip 10pt \hskip
\labelsep{{\normalfont\scshape #1}\savebox\@tempboxa{{\normalfont\scshape #3}}\ifdim
\wd\@tempboxa>\z@ \hskip 5pt\relax {\normalfont\scshape #2}\ \box\@tempboxa\fi.}]
\itshape}
\makeatother

\makeatletter
\renewenvironment{definition}[1][]{\refstepcounter{theorem}\trivlist
  \item[\hskip 10pt\hskip\labelsep{{\normalfont\scshape Definition}\hskip 5pt\relax \thetheorem\if\relax\detokenize{#1}\relax
      .\else
      \hskip 5pt\relax{\normalfont\itshape #1}.\fi
  }]\normalfont\ignorespaces
}{\endtrivlist}

\renewenvironment{remark}[1][]{\refstepcounter{theorem}\trivlist
  \item[\hskip 10pt\hskip\labelsep{{\normalfont\scshape Remark}\hskip 5pt\relax \thetheorem\if\relax\detokenize{#1}\relax
      .\else
      \hskip 5pt\relax{\normalfont\itshape #1}.\fi
  }]\normalfont\ignorespaces
}{\endtrivlist}
\makeatother


\newcommand{\1}{\mathbf{1}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Prb}{\mathbb{P}}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator{\Cov}{Cov}
\newcommand{\piopt}{\ensuremath{\pi_\beta^\star}}

\newcommand{\D}{\mathcal{D}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\annotators}{\mathcal{A}}
\newcommand{\F}{\mathcal{F}}

\DeclareMathOperator{\BordaOp}{Borda}

\newcommand{\B}{\BordaOp}

\newcommand{\marginmat}{M}
\newcommand{\ml}{\pi^{\mathrm{ML}}}
\newcommand{\rewardfn}{r}
\newcommand{\rewardfntheta}{\rewardfn_{\theta}}
\newcommand{\rewardfnstar}{\rewardfn^{\star}}
\newcommand{\pibase}{\pi_{\mathrm{base}}}


\newcommand{\ind}[1]{\mathbf{1}_{\{#1\}}}

\newcommand{\tightdisplayspacing}{\setlength{\abovedisplayskip}{7pt plus 1pt minus 1pt}\setlength{\belowdisplayskip}{7pt plus 1pt minus 1pt}\setlength{\abovedisplayshortskip}{6pt plus 1pt minus 1pt}\setlength{\belowdisplayshortskip}{6pt plus 1pt minus 1pt}}

\makeatletter
\g@addto@macro\normalsize{\tightdisplayspacing}
\g@addto@macro\small{\tightdisplayspacing}
\makeatother

\newcommand{\runinhead}[1]{\par\addvspace{0.35\baselineskip}\noindent\textbf{#1}\enspace\ignorespaces
}

\newif\ifcompactroadmaprefs
\compactroadmaprefstrue

\newcommand{\roadmapref}[2]{\ifcompactroadmaprefs
    \Cref{#1}\else
    \hyperref[#1]{Section~\ref*{#1}: #2}\fi
}

\newcommand{\where}[1]{\par\vspace{-\belowdisplayskip}\vspace{-\parskip}\noindent\emph{where }#1}

\newif\ifshowcomments
\showcommentstrue

\ifshowcomments
\newcommand{\ariel}[1]{{\color{red}[Ariel: #1]}}
\newcommand{\ben}[1]{{\color{orange}[Ben: #1]}}
\newcommand{\shirley}[1]{{\color{violet}[Shirley: #1]}}
\newcommand{\itai}[1]{\textcolor{teal}{[Itai: #1}]}

\newcommand{\sam}[1]{\textcolor{cyan}{[Sam Taggart: #1}]}


\newcommand{\evi}[1]{\textcolor{blue}{Evi: #1}}
\newcommand{\daniel}[1]{\textcolor{magenta}{Daniel: #1}}
\newcommand{\todo}[1]{\textcolor{red}{[TODO: #1]}}
\else
\newcommand{\ariel}[1]{}
\newcommand{\ben}[1]{}
\newcommand{\shirley}[1]{}
\newcommand{\itai}[1]{}
\newcommand{\evi}[1]{}
\newcommand{\daniel}[1]{}
\newcommand{\todo}[1]{}
\fi

\renewcommand{\citet}[1]{\citeauthor{#1}~\citep{#1}}

\newcommand{\barpercent}[1]{\pgfmathsetmacro{\percentvalue}{#1*100}\begin{tikzpicture}[x=1ex,y=1.5ex,baseline]
    \fill[custombar] (0,0) rectangle (#1*10,1);
    \draw[black] (0,0) rectangle (10,1);
    \node[right] at (10.5,0.5) {\small\textbf{\pgfmathprintnumber[fixed,precision=0]{\percentvalue}\%}};
  \end{tikzpicture}}

\tcbset{
  respbox/.style={
    colback=highlightcolor,
    colframe=black!25,
    boxrule=0.6pt,
    arc=2pt,
    left=6pt,
    right=6pt,
    top=4pt,
    bottom=4pt
  }
}

\newcommand{\respbox}[3]{\begin{tcolorbox}[respbox, title=Round #1\\reward: #2]
    \scriptsize #3
  \end{tcolorbox}}

\lstdefinestyle{llm}{
  basicstyle=\ttfamily\footnotesize,
  breaklines=true,
  breakatwhitespace=true,
  columns=fullflexible,
  keepspaces=true,
  showstringspaces=false,
  escapeinside={(*@}{@*)}
}

\newtcolorbox{LLMBox}[2][]{enhanced,
  breakable,
  colback=white,
  colframe=black!35,
  boxrule=0.5pt,
  arc=1mm,
  left=1.5mm,
  right=1.5mm,
  top=1.0mm,
  bottom=1.0mm,
  title=\textbf{#2},
  fonttitle=\normalsize,
  before upper={\ttfamily\footnotesize
    \setlength{\parindent}{0pt}\setlength{\parskip}{0pt}\raggedright
  },
  #1
}


\newcommand{\reward}[2][]{\if\relax\detokenize{#1}\relax
    \rewardfn\!\left(#2\right)\else
    \rewardfn_{#1}\!\left(#2\right)\fi
}

\newcommand{\rewardstar}[2][]{\if\relax\detokenize{#1}\relax
    \rewardfn^{\star}\!\left(#2\right)\else
    \rewardfn_{#1}^{\star}\!\left(#2\right)\fi
}

\newcommand{\rewardtheta}[1]{\reward[\theta]{#1}}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}

